Trustworthy and Secure Service-Oriented Architecture for the Internet of Things

In the Internet of Things (IoT), heterogeneous devices connect to each other and to external systems to exchange data and provide services. Given the diversity of devices, it is becoming increasingly common to establish collaborative relationships between devices to provide composite services. However, due to the high degree of heterogeneity in the IoT context, one of the most significant challenges is to develop software applications that can run on a wide variety of devices and can communicate and collaborate with an even wider array of systems. A common middleware infrastructure for these devices will therefore have a significant impact on the design, deployment, and use of services in IoT systems by allowing developers to focus on the applications rather than the low-level implementation details each device.

==> Outlines.tex <==
Introduction:
IoT has hetergonuese devices 
Middleware is a good way to hide all the abstractions from developer
x,y,z proposed this architecture 
SOA is a good candidate due to its felixibility, easy to integrate new technology,....
but no security or trust 

Security and Trust in IoT
we have see that security is critical because people could die if you dont have it  (IoT device got hacked)
these are various threats we need to protect our devices and middleware agains bad applications, an application should be able to access specific features of the device 
we need to provide a mechanism through which applications can establish the trustworthness of the middleware

Enhanced Architecture 
Picture 
security:
Security policy (describtion)
simillar to android, applications have permissions to access various services
application allowed to check the position of the arm but not move it 

application identification such as using signature 

Policy engine in service managment (policy decision point, Policy data base)
Policy enforcement point - enforce the decision, you are allowed, which services to access 
Device Policy enforcement in the device service proxy 
policy decision point - a lot of information, look at the application, properties, .... and make decision
application Identification:
trust:
Device identification 
middleware attestation.



conclusion and future work 
attestation 








